Online Experimental Design With Estimation-Regret Trade-off Under Network Interference

Network interference has attracted significant attention in the field of causal inference, encapsulating various sociological behaviors where the treatment assigned to one individual within a network may affect the outcomes of others, such as their neighbors. A key challenge in this setting is that standard causal inference methods often assume independent treatment effects among individuals, which may not hold in networked environments. To estimate interference-aware causal effects, a traditional approach is to inherit the independent settings, where practitioners randomly assign experimental participants into different groups and compare their outcomes. While effective in offline settings, this strategy becomes problematic in sequential experiments, where suboptimal decision persists, leading to substantial regret. To address this issue, we introduce a unified interference-aware framework for online experimental design. Compared to existing studies, we extend the definition of arm space by utilizing the statistical concept of exposure mapping, which allows for a more flexible and context-aware representation of treatment effects in networked settings. Crucially, we establish a Pareto-optimal trade-off between estimation accuracy and regret under the network concerning both time period and arm space, which remains superior to baseline models even without network interference. Furthermore, we propose an algorithmic implementation and discuss its generalization across different learning settings and network topology.

==> 2-Preliminary_overview.tex <==




\paragraph{Motivation example} Some scenarios are common and essential, but few have been explored in practice; for example, in pandemic diseases (COVID-19, People may spread the virus to each other), we would like to design strategies and estimators that optimize the patients' welfare and the efficacy of drug effect estimation \textit{simultaneously}.




\paragraph{Overview of our results} Our contributions are summarized as follows:
\begin{itemize}
    \item \textbf{A unified framework.} We propose a unified framework for MAB with interference. We first establish a general interference-based MAB lower bound as a \textit{negative result to motivate the necessity} of reducing the action space. Specifically, we adopt the representation tool, so-called exposure mapping in statistics literature~\citep{leung2022causal, aronow2017estimating}, and encapsulate the regret of the only two articles exploring interference-based bandit~\citep{jia2024multi,agarwal2024multi} as the particular case. 
    
    Our framework is generic primarily because it is flexible. Exposure mapping uses network topology to map the original exponential action space ($ K^N$, $K$ is the arm number; $N$ is the node size) into any (low-dimensional) space of interest.
    Since an oversized action space in an interference-based bandit is unavoidable, our framework concretely exhibits a ``no-free lunch'' scenario: we could arbitrarily manually balance the sacrifice of reward information on the total action space, and the bless of computational efficiency improvement in the algorithm.



Moreover, our model establishes the weakest model assumptions to date, as compared to~\citet{{jia2024multi,agarwal2024multi}}. Our assumptions are inherently verifiable and adjustable, as they are only relevant for the manual definition of network topology and exposure mapping. In other words, for any network topology, we have legitimate exposure map definitions that make the assumption hold.

    \item \textbf{Trade-off between inference and regret.} We bridge the trade-off between the inference in \textit{causality statistics} (i.e., reward gap between arms in bandits or saying average treatment effect (ATE) in causality) and the regret efficiency in \textit{online learning}. 
    
    Informally, we demonstrate that in the stochastic settings, the product \{$\sqrt{\text{regret}}$ $\times$ estimation error\} exhibits a constant order w.r.t. period $T$. In other words, for any given \{policy, estimator\}, we prove a hard instance always exists such that the above product is $\Omega(\sqrt{\vert{\mathcal{U}_{\mathcal{E}}\vert}})$. Stepping forwards, we further demonstrate the above pair \{policy, estimator\} is ``Pareto Optimal'' if and only if the above product is $ O(\sqrt{{\vert\mathcal{U}_{\mathcal{E}}\vert}})$ under all kinds of feasible MAB instances. It is a valid extension of the trade-off currently discussed in~\citet{simchi2023multi, liang2023experimental}, whereas they only specify on the no-interference case. 
    
    \item \textbf{The achievement of Pareto optimality trade-off.} We improve and generalize the UCB algorithm to achieve the above-mentioned Pareto optimality. Specifically, we provide the high probability bound both for the inference and regret.
    \item \textbf{Extension to the adversarial setting.} We further extend the stochastic setting to the adversarial setting. Specifically, our method fully covers~\citet{simchi2023multi,jia2024multi}'s adversarial setting discussion, respectively. Additionally, we also establish the any-time valid confidence sequence for each arm's reward.





    
\end{itemize}




























\begin{table}[t]
\scalebox{0.85}{
\begin{tabular}{cccc}
\hline
    & Estimation  & Regret & Trade-off between Estimation\&Regret \\
    \hline
    Without interference & Traditional causality & Traditional bandit & {\makecell[c]{\citet{liang2023experimental}\\ \citet{simchi2023multi}} }\\
     With interference & {\makecell[c]{{\citet{leung2023network,leung2022causal}} }}& \makecell[c]{\citet{agarwal2024multi} \\ \citet{jia2024multi}} & \textbf{Our paper}\\
     \hline
\end{tabular} }
\caption{The contribution of our paper.}
\end{table}




\paragraph{Future work} Concluding the above, due to the flexibility of exposure-based modeling, the stability of the theoretical optimal balancing guarantee, and the scenario extensibility, our work will be promising in the future to solve the following problems: 
\begin{itemize}
    \item[1] Extension to RL: RL where states are with complex network topology, such as factorized RL, along with the short-long-term problem;
    \item[2] Bandit variants: The neural bandit problem and the GNN fitting model.
    \item[3] Sociological considerations: Preference/human feedback, prospect theory, spatial-temporal interference, Game theory etc. 
\end{itemize}  






